On the Complexity of Reachability Properties in Serverless Function Scheduling

Functions-as-a-Service (FaaS) is a Serverless Cloud paradigm where a platform manages the execution scheduling (e.g., resource allocation, runtime environments) of stateless functions. Recent developments demonstrate the benefits of using domain-specific languages to express per-function scheduling policies, e.g., enforcing the allocation of functions on nodes that enjoy low data-access latencies thanks to proximity and connection pooling. We present aAPP, an affinity-aware extension of a platform-agnostic function scheduling language. We formalise its scheduling semantics and then study the complexity of statically checking reachability properties, e.g., useful to verify that trusted and untrusted functions cannot be co-located. Analysing different fragments of aAPP, we show that checking reachability of policies without affinity has linear complexity, while affinity makes the problem PSpace.

==> app_encoding.tex <==
\section{\app encoding}

\todo[inline]{mettere tutto quanto serve per la semantica di app e appp. Copia incolla dal papero ECOOP fissando i problemi trovati da Save}
We assume that \app scripts \emph{a}) include the policy
``$\mathtt{default}\hlstr{:}\ \texttt{-}\ \hln{workers}\ :\ \hlopt{*}$'' unless
the user customises the \texttt{default} policy and \emph{b}) show the \texttt{default} policy as the last one in order of appearance.

\label{sec:encoding}
\begin{figure}[h]
\begin{adjustbox}{width=.9\textwidth}
\begin{minipage}{\textwidth}
{\footnotesize
\[
  \enc{\many{-\ \textit{tag}} \ ::\ -\ \mathtt{default}\hlstr{:} \many{\mathtt{-}\ \textit{block}}}
  = \enc{\many{-\ \textit{tag}} \ ::\ -\ \mathtt{default}\hlstr{:} \many{\mathtt{-}\ \textit{block}}
  \quad \hln{followup} \hlstr{:}\ \hlopt{fail}}
\]
\[
  \begin{array}{rll}
    \enc{\many{-\ \textit{tag}} \ ::\ -\ \mathtt{default}\hlstr{:} \many{\mathtt{-}\ \textit{block}}
    \quad \hln{followup} \hlstr{:}\ \fopt}
    & = & \bigcup\limits_{t \ \in\ \many{\textit{tag}}} \left\{\enc{t}_{\many{\enc{\textit{block}}}}\right\}
  \\
  \enc{\textit{id} \ \hlstr{:} \ \many{\mathtt{-}\ \textit{block} }}_{\many{\block}} =
  \enc{\textit{id} \ \hlstr{:} \ \many{\mathtt{-}\ \textit{block} } \quad
    \hln{followup}\ \hlstr{:}\ \hlopt{default}}_{\many{\block}} & = &
    (\textit{id}, \many{\enc{\textit{block}}} :: \many{\block})
  \\[.5em]
  \enc{\textit{id} \ \hlstr{:} \ \many{\mathtt{-}\ \textit{block} } \quad
    \hln{followup}\ \hlstr{:}\ \hlopt{fail}}_{\many{\block}} & = &
    (\textit{id}, \many{\enc{\textit{block}}})
    \\
    \enc{\hln{workers} \hlstr{:}\ \wopt}
    & = & ( \enc{\textit{\wopt}}, \hlopt{any}, \hlopt{capacity\_used}\ 100\hlopt{\%}::\emptyseq)
    \\
    \enc{\hln{workers} \hlstr{:}\ \wopt
    \quad \hln{strategy} \ \hlstr{:}\ \sopt}
    & = & ( \enc{\wopt}, \sopt, \hlopt{capacity\_used}\ 100\hlopt{\%}::\emptyseq )
    \\
    \enc{\hln{workers} \hlstr{:}\ \wopt
      \quad \hln{invalidate} \ \hlstr{:}\ \many{-\ \iopt}}
    & = & ( \enc{\wopt}, \hlopt{any}, \many{\iopt} )
    \\
    \enc{\hln{workers} \hlstr{:}\ \wopt
      \quad \hln{strategy} \ \hlstr{:}\ \sopt
      \quad \hln{invalidate} \ \hlstr{:}\ \many{-\ \iopt}}
    & = & ( \enc{\wopt}, \sopt, \many{\iopt} )
    \\
    \enc{\hlopt{*}} & = & \hlopt{*}
    \\
    \enc{\many{-\ id}} & = & \many{\ id}
    \\
  \end{array}
\]
}
\end{minipage}
\end{adjustbox}
\caption{\app Syntax Encoding.}
\label{fig:encoder}
\end{figure}

The encoding function $\enc{\cdot}$ translates an \app script into a policy
function. The encoding, reported in \cref{fig:encoder}, is straightforward: we
inductively walk through the syntax of the \app script and translate each
fragment into the corresponding mathematical object in \(\Policies\).
%
The only notable bits regard the inclusion of the standard options for the
missing parameters---for \hln{strategy} we set it to \hlopt{any} and for
\hln{invalidate} we set it to the maximal capacity of the worker, i.e.,
\hlopt{capacity\_used}\ 100\hlopt{\%}---and the static resolution of the
\hln{followup} parameter, where we concatenate the list of blocks of the tag with
the blocks of the \code{default} one, in case the \hlopt{default} option is
present. Notation-wise, we introduce \(::\) and \(\emptyseq\) to resp.
indicate list concatenation and empty sequence (frequently omitted for brevity).


\section{\appp Encoding}
\label{sec:encoding_appp}
We define the encoding function \(\encp{\cdot}\) to translate \appp{} scripts into the extended mathematical representation of policy functions. In \cref{fig:encoder_appp}, we report the encoding function \(\encp{\cdot}\) from
the syntax to the objects used in the operational semantics. The interesting bit in the definition of \(\encp{\cdot}\) is the revision of the block-encoding rule (third from the bottom). The rule reuses the related rule in \cref{fig:encoder} (\(\enc{\cdot}\)) to encode the fragments already present in \app and it hands the encoding of the new \hln{affinity} clause to the rules \(\encp{\cdot}_{+}\) and \(\encp{\cdot}_{-}\) resp.\ for the affine and anti-affine tags.

\begin{figure}[h]
\begin{adjustbox}{width=.76\textwidth}
\begin{minipage}{\textwidth}

\[
  \encp{\many{-\ \textit{tag}} \ ::\ -\ \textit{default}\ \hlstr{:} \many{\mathtt{-}\ \textit{block}}}
  = \encp{\many{-\ \textit{tag}} \ ::\ -\ \textit{default}\ \hlstr{:} \many{\mathtt{-}\ \textit{block}}
  \quad \hln{followup} \hlstr{:}\ \hlopt{fail}}
\]
\[
  \begin{array}{rll}
    \encp{\many{-\ \textit{tag}} \ ::\ -\ \textit{default}\ \hlstr{:} \many{\mathtt{-}\ \textit{block}}
    \quad \hln{followup} \hlstr{:}\ \fopt}
    & = & \bigcup\limits_{t \ \in\ \many{\textit{tag}}} \left\{\encp{t}_{\many{\encp{\textit{block}}}}\right\}
  \\
  \encp{\textit{id} \ \hlstr{:} \ \many{\mathtt{-}\ \textit{block} }}_{\many{\beta}} =
  \encp{\textit{id} \ \hlstr{:} \ \many{\mathtt{-}\ \textit{block} } \quad
    \hln{followup}\ \hlstr{:}\ \hlopt{default}}_{\many{\beta}} & = &
    (\textit{id}, \many{\encp{\textit{block}}} :: \many{\beta})
  \\[.5em]
  \encp{\textit{id} \ \hlstr{:} \ \many{\mathtt{-}\ \textit{block} } \quad
    \hln{followup}\ \hlstr{:}\ \hlopt{fail}}_{\many{\beta}} & = &
    (\textit{id}, \many{\encp{\textit{block}}})
  \end{array}
\]
\[
  \begin{array}{rll}
    \encp{\textit{block}} & = & \begin{cases}
      (\wopt,\sopt,\many{\iopt},\emptyseq,\emptyseq) &
        \mbox{if } \enc{\textit{block}} = (\wopt,\sopt,\many{\iopt})
      \\[1em]
      (\wopt,\sopt,\many{\iopt},\encp{\many{\textit{\aopt}}}_{+}, \encp{\many{\textit{\aopt}}}_{-}) &
        \mbox{otherwise, let } \textit{block} = \mbox{``}\bullet \quad \hln{affinity} \ \hlstr{:}\ \many{-\ \textit{\aopt}}\ \mbox{''} \\ & \mbox{and} \ \enc{\bullet} = (\wopt,\sopt,\many{\iopt})
    \end{cases}
    \\
      	\encp{\emptyseq}_{\bullet} & = & \emptyseq
	\\
    \encp{\aopt :: \many{\aopt}}_{\bullet} & = &
    \begin{cases}
      id :: \encp{\many{\aopt}}_{\bullet} &
      \mbox{if } ( \aopt = \textit{id} \ \wedge \ \bullet = + )
      \vee ( \aopt = \textit{!id} \ \wedge \ \bullet = - )
%    \\
%    \emptyseq & \mbox{if } \many{\aopt} = \emptyseq
    \\
    \encp{\many{\aopt}}_{\bullet} & \mbox{otherwise}
  \end{cases}
  \end{array}
\]
\end{minipage}
\end{adjustbox}
\caption{\appp
% updated structure for \textit{block}s (\(\Blocks\)) and
% dedicated
encoding.}
\vspace{-1em}
\label{fig:encoder_appp}
\end{figure}




% : we first consider the encoding ${\many{\block}}$ of the
% blocks in the \texttt{default} tag (which we assume
% to always appear as the last element of an \textit{app} script) and then the encoding
% of the other custom tags continues with a reference to ${\many{\block}}$
% (with the signature \(\enc{\cdot}_{\many{\block}}\)). In this way, it is possible
% to append the blocks $\many{\block}$ to custom tags having the \hl{followup} strategy
% \hlopt{default}.



%We define the encoding $\enc{\cdot}$ inductively on the syntax of APP scripts
%(see \cref{fig:app_syntax}). The encoding statically resolves the followup
%strategy. In the rules, we first separate the encoding of the custom tags (in
%\textit{app}) from the \texttt{default} one (which we assume to always appear as
%the last element of an \textit{app} program), so that the encoding continues
%with a reference to the blocks belonging to the \texttt{default} tag (with the
%signature \(\enc{\cdot}_{\many{\block}}\)). When resolving a tag, if the
%\hl{followup} strategy is \hlopt{default}, we associate the \textit{policy\_tag}
%with the encoding of its related \textit{block}s, followed by the ones of the
%\code{default} tag, carried in \(\many{\block}\); if the \hl{followup} strategy
%is \hlopt{fail} we associate the \textit{policy\_tag} only to the encoding of
%its \textit{block}s. The notation \((\textit{policy\_tag}, \many{\block})\)
%identifies a pair associating one tag to a list of policy blocks (we use $\cup$
%to assemble the pairs into a function from tags to blocks). The other rules of
%\cref{fig:encoder} are straightforward. We skip their piecemeal comment and
%rather


==> encoding.tex <==
\section{Automated verification of \appp scripts}
\label{sec:pddl_encoding}

%\todo[inline]{
% \begin{itemize}
%   \item Vogliamo implementare un analizzatore di reachabiliy e co-occurrence
%   \item Invece di implementare un nostro algoritmo ad-hoc, abbiamo deciso di utilizzare
%         solver disponibili in letteratura
%   \item I solver piu' vicini alle nostre esigenze sono i PLANNER che risolvono in modo
%         costruttivo problemi di reachability (costruttivo, in quanto restituiscono la traccia
%         che permette di raggiungere lo stato target).
%   \item Tali solver richiedono la specifica del problema da risolvere in un linguaggio dedicato
%         chiamato PDDL.
%   \item La tipica specificia PDDL, si divide in due parti (i) domain description (e.g. descrive le
%         possibili azioni indicandone le preconditions e gli effects) e (ii) problem description (e.g. include
%         la specifica delle initial conditions e dei goals).
%   \item Il nostro approccio e' stato quello di encodare la semantica operazionale di \appp come domain description, mentre la configurazione, l'\appp script e lo specifico problema di reachability/co-occurrence vengono specificati come problem description.
%   \item Dire semplicemente che il nostro dominio encoda la semantica operazionale (le azioni coincidono con le transizioni dell'LTS) e mettere i sorgenti in appendice.
% \end{itemize}
%}

Given the definition of the \Reach~ and \CoOccur~ problems and the related
results for \app and \appp, we have a firmer grasp of how to automate their
analysis, provided an initial configuration. Since we proved that the complexity
of this analysis for \appp is PSPACE-hard, we present a proof-of-concept
solution developed on existing solvers for that class of problems. 

Specifically, we encode the \Reach~ and \CoOccur~problems as automated planning
tasks, and we choose to use PDDL~\cite{FL03}, i.e., the de-facto standard for
encoding planning problems. PDDL specifications typically include two parts. A
domain description and a problem description. The domain regards all available
actions, each with its preconditions and effects. The problem concerns the
initial state for the specific problem instance, along with the desired goals.

The choice of PDDL has many advantages, the main ones include: \emph{i}) it lets
us use different dedicated and efficient planning solvers, \emph{ii}) it
naturally provides a witness (i.e., a sequence of actions) leading to the
violation of some desired property (e.g., if two functions shall be anti-affine
and we find an instance where they co-occur, we can see a trace that produces
the offending result), and \emph{iii}) it lets users express more
elaborate goal configurations than reachability and co-occurrence (i.e.,
we can check if a given configuration is reachable).

\subsection{Encoding of the PDDL domain}
To define the domain, we encoded the semantic rules reported in
\cref{fig:rules,fig:rules_app_plus}. The two main encoded actions are the
\textit{(start, \_, \_)} and \textit{(done, \_, \_)} transitions.
%, using the rules as preconditions.
Each action alters the state appropriately, e.g., removing a function from a
worker increases its available capacity accordingly. The encoding of the rules
uses a combination of boolean predicates (e.g., for the affinity of a block) and
numerical functions (e.g., for capacity constraints). We did not encode the
\textit{(fail, \_, \_)} transition since it does not affect the state%
% and would loop back to the previous configuration
---it is equivalent to a null operation in the context of a plan.

\subsection{Encoding of the PDDL problems}

Since \appp's semantics works on \appp scripts and configurations (cf.
\cref{fig:rules,fig:rules_app_plus}), we define the problem by encoding an input
\appp script with a companion configuration definition, which describes the
existing workers and functions with the respective capacities/occupancies---the
latter, defined using PDDL \emph{numeric fluents}, which model non-binary,
discrete resources. Given a configuration, we set the initial state such that
workers have no allocated functions and maximal capacity. Finally, we define the
\Reach~ and \CoOccur~ problems using of the proposition
\textit{number\_of\_f\_in\_W}, which indicates the number of copies of a function
%\textit{f} 
on a given %the
worker %\textit{w} 
in the final state. The code on the left of \cref{fig:pddl_prop_examples}
exemplifies the \Reach~ problem, where we check if we can satisfy the \hln{goal} of allocating at least one copy of function \texttt{f} on worker
\texttt{w}; on the right of \cref{fig:pddl_prop_examples}, we realise \CoOccur~
as the conjunction of two \textit{number\_of\_f\_in\_W}, checking if worker
\texttt{w} can host both functions \texttt{f1} \texttt{and} \texttt{f2}.

% It has to be noted that while only \Reach~ and \CoOccur~ have been analysed in this work, PDDL allows us to describe more complex and versatile goals,
% such as the one used in \cref{subsec:example_pddl_app}.

\begin{figure}
  \begin{adjustbox}{width=.99\textwidth}
    \hspace{2em}
    \begin{minipage}{.52\linewidth}
      \begin{codeEnv}
        \vspace{.55em}
        \begin{lstlisting}[xleftmargin=-1em,language=Lisp,basicstyle=\footnotesize\ttfamily]
(:goal
  (= (number_of_f_in_W f w) 1)
)
\end{lstlisting}
        \vspace{.55em}
      \end{codeEnv}
    \end{minipage}
    \hspace{1em}
    \begin{minipage}{.6\linewidth}
      \begin{codeEnv}
        \begin{lstlisting}[xleftmargin=-1em,language=Lisp,basicstyle=\footnotesize\ttfamily]
(:goal
  (and (= (number_of_f_in_W f1 w) 1)
       (= (number_of_f_in_W f2 w) 1)
))
\end{lstlisting}
      \end{codeEnv}
    \end{minipage}
  \end{adjustbox}
  \vspace{-1em}
  \caption{Encoding of \Reach~ and \CoOccur~ in PDDL, on the left and right side respectively.\vspace{-1.5em}}
  \label{fig:pddl_prop_examples}
\end{figure}

\subsection{Tool Components and Support for Advanced Queries, an Example} \label{subsec:example_pddl_app}

%To test our encoding, we defined a scenario, where we want to check whether a given
% \appp script allows a specific unwanted scenario to happen. We named this scenario "\textit{singleton}",
% as the main goal is to prevent a given function from ever co-occurring with any other function,
% on any worker.

To provide a smoother experience to users, we equipped our PDDL encoding with a
simple, YAML-like notation for configurations (exemplified in
\cref{fig:ex_configuration}) and translators that generate the PDDL encoding of
part of the problem, given a configuration file and an \appp script. The last
piece of the problem, required from the user, is the definition of the
\hln{goal}, which uses the PDDL notation. The encoding and its companion tools
are available at~\cite{repository_pddl}.

To illustrate the experience of using our analysis tool, we exemplify the
definition of a configuration, an \appp script, and a property.
%
Let us consider the configuration in \cref{fig:ex_configuration}, with two
workers, \texttt{local} and \texttt{public}, and three functions \texttt{f},
\texttt{u} and \texttt{g}, resp. tagged \texttt{private}, \texttt{unsafe}, and
\texttt{generic}. We want to define an \appp script such that \emph{it never
happens that we allocate \texttt{f}s with other non-\texttt{f} functions}. We
encode this property in \cref{fig:ex_predicate}, where we use the existential
quantifiers to range over both workers and functions and check whether we can
find a worker that can host both \texttt{f} and a function different from
\texttt{f}. If the planner is unable to find a solution, the property holds for
the provided \appp script and configuration.

%
% \begin{figure} \begin{minipage}{.45\linewidth}
%   \begin{lstlisting}[basicstyle=\tiny\ttfamily] workers: - name: local
%   capacity: 20 - name: public capacity: 20 functions: - name: f tag: private
%   capacity: 5 - name: u tag: unsafe capacity: 5 - name: g tag: generic
%   capacity: 5 \end{lstlisting} \caption{Environment configuration for the
%   \textit{singleton} example.} \label{fig:pddl_example_env} \end{minipage}
%   \hfill \begin{minipage}{.45\linewidth}
%   \begin{lstlisting}[basicstyle=\tiny\ttfamily] (:goal (exists (?w - worker
%   ?f2 - function) (and (not (= ?f2 f)) (= (amount_f_in_W f ?w) 1) (=
%   (amount_f_in_W ?f2 ?w) 1)
%         )
%     )
%   )
%   \end{lstlisting} \caption{PDDL encoding of the goal for the
%     \textit{singleton} example.} \label{fig:pddl_example_goal} \end{minipage}
%     \end{figure}
%
In \cref{fig:ex_app_script}, we show a possible candidate script. However,
running the planner with (the encodings of) the excerpts in
\cref{fig:ex_configuration} and \cref{fig:ex_app_script} and the goal from
\cref{fig:ex_predicate}, we obtain the output in the red box in the bottom of \cref{fig:ex_predicate}. The output is a trace of actions that satisfies the
goal; namely, the allocation of \texttt{f} with another function on the same
worker. Specifically, we found that \texttt{f} can co-occur with a function
\texttt{g}, tagged \texttt{generic}, on the \texttt{local} worker. Hence, we
need to fix our candidate \appp script to prevent the allocation of
\texttt{generic} functions with \texttt{f}s. 
%
% A possible \appp script for this configuration is shown in
% \cref{fig:ex_app_script_fixed}, where we use anti-affinity to specify that
% \textit{private} functions should not be scheduled with any other. When
% encoding this as a PDDL problem, the output of the planner shows that the
% given script is incorrect since there exists a valid sequence of actions
% ending in a state that satisfies the goal. Indeed, as shown in the red box
% under \cref{fig:ex_predicate}, the \textit{generic} function was scheduled on
% the \textit{local} worker, together with the \textit{private} function.
%
\input{pddl_example}
%
% From the generated plan, it can be seen how \textit{f} (i.e., the
% \textit{private} function) is successfully scheduled on the empty
% \textit{local} worker in step 0, thereby satisfying its affinity and location
% constraints. On the other hand, \textit{g} (i.e., the \textit{generic}
% function) is scheduled right after on the same worker in step 1, apparently
% violating these same affinity constraints. 
Looking closely at \cref{fig:ex_app_script}, we notice that we forgot to
indicate that also the \texttt{generic} (tagged) functions are anti-affine with
the \texttt{private} ones. Remember that \hln{affinity} in \appp is not
symmetric, so, to ensure that \texttt{private} functions are anti-affine with
the other functions, we need to mark also all the latter anti-affine with the
\texttt{private} ones. 
% each other indeed co-occur with \textit{generic} ones, simply by scheduling
% the latter after the former.

\cref{fig:ex_app_script_fixed} shows a fixed version of the \appp script from
\cref{fig:ex_app_script}, where we added a new \hln{affinity} clause under the
\texttt{generic} block. The additional constraint is enough to make the goal
from \cref{fig:ex_predicate} unsatisfiable, as shown in the green box on the
right of \cref{fig:ex_app_script_fixed}.

%\subsection{Implementation details}

Performance-wise, we tested our encoding using the
MetricFF~\cite{hoffmann:ecai-02} planner on examples like the previous one,
%  from
% \cref{fig:pddl_example}, 
obtaining results (either providing a solution or
proving its non-existence) within a few milliseconds---specifically, we obtain a
solution in 2.4ms for the script in \cref{fig:ex_app_script} and the exhaustion
for the one in \cref{fig:ex_app_script_fixed} in 4ms, averaged over \(10^4\)
runs.

Here, we focus on the feasibility of our approach based on using off-the-shelf
planning solvers, hence we leave as future work the study of which planners work
best and how well they scale under different cases. Like SAT solvers, which can
solve large SAT problems despite their NP-hardness, we conjecture that planners
can efficiently solve the majority of realistic 
%  the reachability and co-occurrence
problems. Intuitively, except for those combinations of configuration, script,
and predicates that require the saturation of workers to reach the goal, the
plan to prove the violation of the property is rather short and therefore
solvers can find it quickly.\footnote{Note also that the complexity of the
planning problem becomes trivially pseudo-polynomial when the maximal length of
the plan is bound (i.e., $O(n^k)$ where $n$ is the size of the planning encoding
and $k$ is the maximal length of the allowed plan).}

==> pddl_example.tex <==
\begin{figure}
\begin{adjustbox}{width=\textwidth}
\noindent\begin{minipage}[t]{.22\textwidth}
\vspace{-1.8em}
% \begin{center}Configuration\end{center}
\caption{Workers and functions\label{fig:ex_configuration}.}
\begin{adjustbox}{width=\textwidth}
\begin{minipage}{1.1\textwidth}
\begin{codeEnv}
\begin{lstlisting}[xleftmargin=-1em,mathescape,numbers=left,basicstyle=\footnotesize\ttfamily,numberstyle=\tiny]
$\hln{workers}$:
  - name: local
    capacity: 20
  - name: public
    capacity: 20
$\hln{functions}$:
  - name: f
    tag: private
    occupancy: 5
  - name: u
    tag: unsafe
    occupancy: 5
  - name: g
    tag: generic
    occupancy: 5
\end{lstlisting}
\end{codeEnv}
\end{minipage}
\end{adjustbox}
\end{minipage}
    %
\begin{minipage}[t]{.10\textwidth}
\begin{tikzpicture}[baseline=(current bounding box.north)]
\draw[white] (0,0) rectangle (0,6.2);
\draw[decoration={brace,aspect=0.75,amplitude=10pt,mirror},decorate](0,0) -- (0,6);
\draw[->] (.5,4.5) -- (1,4.5);
\end{tikzpicture}
\end{minipage}
\hspace{-.5em}\begin{minipage}[t]{.39\textwidth}
\vspace{-1.8em}
\caption{Checker predicate\label{fig:ex_predicate}.}
% \begin{center}Checker predicate\end{center}
\begin{adjustbox}{width=\textwidth}  
\begin{minipage}{1.15\textwidth}
\begin{codeEnv}
\begin{lstlisting}[
  xleftmargin=-1.1em,
  language=Lisp,
  basicstyle=\footnotesize\ttfamily,
]
(:goal
 (exists 
  (?w - worker ?f2 - function)
  (and (not (= ?f2 f))
   (=(number_of_f_in_W f ?w)1)
   (=(number_of_f_in_W ?f2 ?w)1)
)))
\end{lstlisting}
\end{codeEnv}
\end{minipage}
\end{adjustbox}
\vspace{-1.5em}
\begin{center}
\begin{tikzpicture}[baseline=(current bounding box.north)]
  \draw[->] (0,.5) -- (0,0);
\end{tikzpicture}
\end{center}
\begin{adjustbox}{width=\textwidth}  
\begin{minipage}{1.1\textwidth}
\begin{codeEnv}[red!10!white]
\begin{lstlisting}[basicstyle=\footnotesize\ttfamily]
step
  0: ADD_F_TO_W_WITH_BLOCK 
      F LOCAL PRIVATE_B0
  1: ADD_F_TO_W_WITH_BLOCK 
      G LOCAL GENERIC_B0
  2: REACH-GOAL
\end{lstlisting}
\end{codeEnv}
\end{minipage}
\end{adjustbox}
\end{minipage}
    \begin{minipage}[t]{.10\textwidth}
      \begin{tikzpicture}[baseline=(current bounding box.north)]
        \draw[white] (0,0) rectangle (0,6.2);
        \draw[<-] (0,4.5) -- (.5,4.5);
        \draw[decoration={brace,aspect=0.779,amplitude=10pt},decorate](1,.3) -- (1,5.7);
      \end{tikzpicture}
    \end{minipage}
    \hspace{-1em}\begin{minipage}[t]{.22\textwidth}
      % \begin{center}APP script\end{center}
      \vspace{-1.8em}
      \caption{\appp script\label{fig:ex_app_script}.}
      \vspace{1em}
% \hspace{-2em}
\begin{minipage}{\textwidth}
\begin{adjustbox}{width=\textwidth}  
\begin{minipage}{1.05\textwidth}
\begin{codeEnv}
\begin{lstlisting}[xleftmargin=-1em,xrightmargin=-1em,language=yaml,mathescape,basicstyle=\footnotesize\ttfamily,numbers=right,numberstyle=\tiny]
- private:
  - $\hln{workers}$:
      - local
    $\hln{affinity}$:
      - !unsafe
      - !generic
- unsafe:
  - $\hln{workers}$:
      - public
    $\hln{affinity}$:
      - !private
- generic:
  - $\hln{workers}\hlstr{:}\ \hlopt{*}$
\end{lstlisting}
\end{codeEnv}
\end{minipage}
\end{adjustbox}
\end{minipage}
\end{minipage}
\end{adjustbox}
  
  % \vspace{-.8em}
\hspace{.25\textwidth}\begin{minipage}{.6\textwidth}
  {\vspace{.5em}\color{gray}\phantom{a}\hrule}
\end{minipage}
% \vspace{-.4em}

% \begin{adjustbox}{width=\textwidth}
\begin{minipage}[t]{.58\textwidth}
\vspace{-1em}
\caption{Fixed APP script\label{fig:ex_app_script_fixed}.}
\begin{adjustbox}{width=\textwidth}
\begin{minipage}[t]{1.2\textwidth}
\begin{codeEnv}
\begin{minipage}[t]{.32\textwidth}
\begin{lstlisting}[xleftmargin=-.5em,language=yaml,mathescape,basicstyle=\footnotesize\ttfamily]
- private:
  - $\hln{workers}$:
      - local
    $\hln{affinity}$:
      - !unsafe
      - !generic
\end{lstlisting}
\end{minipage}
\hspace{-.2em}
{\color{yellow!80!black}\vrule}
% \hspace{1em}
\begin{minipage}[t]{.32\textwidth}
\begin{lstlisting}[language=yaml,mathescape,basicstyle=\footnotesize\ttfamily]
- unsafe:
  - $\hln{workers}$:
      - public
    $\hln{affinity}$:
      - !private
\end{lstlisting}
\end{minipage}
\hspace{.7em}
{\color{yellow!80!black}\vrule}
\hspace{-1em}
\begin{minipage}[t]{.32\textwidth}
\begin{lstlisting}[xleftmargin=1em,language=yaml,mathescape,basicstyle=\footnotesize\ttfamily]
- generic:
  - $\hln{workers}\hlstr{:}\ \hlopt{*}$
    $\hln{affinity}$:
     - !private
\end{lstlisting}
\end{minipage}
\end{codeEnv}
\end{minipage}
\end{adjustbox}
\end{minipage}
\begin{minipage}[t]{.08\textwidth}
\vspace{2em}
\begin{center}
\begin{minipage}{.8\textwidth}
  {\tiny   + \cref{fig:ex_configuration}
    \\[-1em] + \cref{fig:ex_predicate}}
\end{minipage}
\end{center}
\vspace{-1em}
\begin{tikzpicture}[baseline=(current bounding box.north)]
\draw[->] (0,0.5) -- (1,.5);
\end{tikzpicture}
\end{minipage}
\begin{minipage}[t]{.33\textwidth}
\vspace{1.1em}
\begin{codeEnv}[green!10!white]
\begin{adjustbox}{width=1.1\textwidth}
\hspace{-1.5em}\begin{lstlisting}[xleftmargin=-1.6em]
Enforced Hill-climbing failed!
switching to Best-first Search now.

advancing to distance: 3

best first search space empty!
problem proven unsolvable.
\end{lstlisting}
\end{adjustbox}
\end{codeEnv}
\end{minipage}
% \end{adjustbox}
% \caption{Example of incorrect \appp script for the \textit{singleton} example
% (top) and fix (bottom).}
% \vspace{-1.5em}
\label{fig:pddl_example}
\end{figure}
